CLEANN: Accelerated Trojan Shield for Embedded Neural Networks

We propose CLEANN, the first end-to-end framework that enables online mitigation of Trojans for embedded Deep Neural Network (DNN) applications. A Trojan attack works by injecting a backdoor in the DNN while training; during inference, the Trojan can be activated by the specific backdoor trigger. What differentiates CLEANN from the prior work is its lightweight methodology which recovers the ground-truth class of Trojan samples without the need for labeled data, model retraining, or prior assumptions on the trigger or the attack. We leverage dictionary learning and sparse approximation to characterize the statistical behavior of benign data and identify Trojan triggers. CLEANN is devised based on algorithm/hardware co-design and is equipped with specialized hardware to enable efficient real-time execution on resource-constrained embedded platforms. Proof of concept evaluations on CLEANN for the state-of-the-art Neural Trojan attacks on visual benchmarks demonstrate its competitive advantage in terms of attack resiliency and execution overhead.

==> 6_related_old.tex <==
\section{Related Work}\label{sec:related}
Since the introduction of Trojan attacks~\cite{gu2017badnets,liu2017trojaning}, developing defense strategies has gained interest. In the following, we provide a complete taxonomy of DNN Trojan mitigations. 


\subsection{Defense by robust training and fine-tuning}
One plausible threat model assumes that the adversary provides a contaminated dataset, leaving training of the model to the attack victim. Pioneer research in robust learning can identify malicious samples during training~\cite{charikar2017learning, liu2017robust,tran2018spectral}. In another line of work, an already-infected DNN is modified by either retraining pruned networks~\cite{liu2018fine} or fine-tuning the model with reverse-engineered Trojan images~\cite{wang2019neural, chen2019deepinspect}, an approached referred as ``patching''. Our threat model is stronger than these works: we assume that the attack victim does not have access to the training dataset.  Additionally, our method does not rely on expensive model retraining to establish the defense.

\subsection{Defense by model and data inspection} 

The attack surface can be investigated after the pretrained malicious model is purchased from the adversary. Mitigation approaches in this track are categorized as follows: (1)~methods that inspect the DNN model, to find out if it is tampered with a backdoor attack, and possibly reverse engineering the trigger. (2)~methods that check the input samples to identify the presence of Trojan triggers, without directly attempting to reverse-engineer the trigger. Our work falls in the second category. Each of the existing work makes different assumptions about access to training data and labels, access to the DNN model, the ability to fine-tune the DNN weights, and prior knowledge about the Trojan attack. In the following, we overview related work in category (1) and (2).

% \subsection{Mitigation at Inference}
\noindent{\bf Mitigation by Trigger Restoring.} Neural Cleanse~\cite{liu2017neural} is an end-to-end framework that searches for possible Trojan trigger patterns in the input domain. The triggers are extracted without access to the training dataset. Follow up work~\cite{chen2019deepinspect} improves the search runtime of Neural Cleanse using generative Adversarial Networks. Authors of~\cite{guo2019tabor} show that their framework can achieve better reverse-engineering on slightly more complex triggers; Though effective in reverse-engineering simple patterns, these methods become futile in finding more complex triggers, e.g., those created by TrojanNN~\cite{liu2017trojaning}. ABS~\cite{liu2019abs} proposes stimulating neurons and studying the model's behavior to extract Trojan triggers. This method makes an implicit assumption about the attack algorithm: that the Trojan is inserted through a single neuron (as in the TrojanNN attack~\cite{liu2017trojaning}). Our method is different than the works in this category in that, instead of reverse engineering the trigger, we study the statistics of benign samples and detect abnormal triggers during inference. This approach allows \sys{} to eliminate complex Trojan trigger patterns without prior knowledge about the attack algorithm. 
\mojan{add other benefit, overhead, etc.}


% \begin{itemize}
%     \item NeuralCleanse~\cite{wang2019neural}: \edit{from TABOR:} Wang et al. [51] propose the first end-to-end trojan detection technique without the above assumptions. They model the trojan restoration as an optimization task and restore the po- tential triggers for all labels. Then they leverage MAD outlier detection method to distinguish the correct trigger.
%     \item DeepInspect~\cite{chen2019deepinspect}: \edit{from TABOR:} Follow- ing [51]’s idea (i.e., using the same objective function and anomaly detection method), Chen et al. [8] further borrow the idea of Generative Adversarial Network [21] to generate the trigger. However, as we show in Section §5, the objective function in [51, 8] cannot restore high-fidelity triggers and the anomaly detection method employed in [51, 8] typically incurs unaffordable false identification rate. \edit{from FeBURUS:} DeepInspect (DI) [10] shows their robustness against backdoor detection and mitigation in strict settings that they do not hold the clean dataset for defense and work in the black- box setting. DI has shown to be faster than Neural Cleanse [44] in the complex dataset for reversing triggers and shows their robustness against advanced backdoor variants such as trigger size or the number of Trojan targets. However, due to the strict assumption of having no access to the clean data , the result of this method is worse than other state-of-the-art defense methods such as [19], [44] with the attack success rates after model patching with reversed dataset and triggers are around 8\%. Even when authors assume to have clean data, the attack success rates are around 3\% which are still higher than other methods such as Neural Cleanse or ours (around 0\%). Detailed comparison of attack success rate of ours vs. the counterparts in the literature is shown in Table VII. In addition, similar to Neural Cleanse [44] or TABOR [19], DI [10] has to change their approach to deal with an adaptive attack like Partial Backdoor.
%     \item TABOR~\cite{guo2019tabor}: \edit{from FEBURUUS:} In TABOR, authors have shown that their method is effective in not only detecting the triggers but also reverse engineer the triggers with the improvement in the fidelity of the reversed triggers compared with Neural Cleanse method \cite{wang2019neural}. However, there are still limitations in this TABOR method such that it cannot address some advanced backdoor variants such as multiple triggers targeted to the same label or partial backdoor.
    
%     \item ABS~\cite{liu2019abs}. \edit{from TABOR:} In [32], Liu et al. propose another trigger restoration technique which does not rely on contaminated training data but still assumes the access to the hidden layer outputs. Another limitation of this work is that it lacks efficient anomaly detection method to determine the existence of trojan backdoor and the target label. \edit{from another paper:} This works makes the assumption that the attack is effective when a single neuron encodes the backdoor. This is a huge assumption about the attack, which is also used by TrojanNN.
% \end{itemize}


\noindent{\bf Mitigation by Input Investigation.} Similar to \sys{} methodology, several contemporary research works aim at eliminating trigger patterns present at the data, without focusing at trigger reverse engineering. \cite{chen2018detecting} suggest querying the infected model and performing activation clustering on the hidden layer features to determine whether a model is infected or not. NIC~\cite{ma2019nic} compares hidden featuremap patterns with legitimate and Trojaned data samples to detect adversaries. These method require having access to the contaminated training dataset or the ratio of the infected samples, \mojan{which might not be realistic.} \sys{}, in contrast, does not require access to the training data or infected data samples to construct the defense. 

% To identify potential trigger patterns in the input, 
Sentinet~\cite{chou2018sentinet} computes a saliency map over the input features, using gradient information obtained by back propagation.  Feburuus~\cite{doan2019februus} proposes a similar approach along with utilizing GANs to replace the candidate trigger patterns with benign content.
STRIP~\cite{gao2019strip} runs the model multiple times on the image with intentional injected noise, to identify Trojaned samples. The above defenses are established using unlabeled clean data, with the caveat that the number of data samples required for GAN training might be large. 
The detection accuracy of these works is shown to be high; however, their computational burden makes them unsuitable for embedded applications since multiple rounds of forward and backward propagation are required per input. \mojan{\sys{} achieves a better detection accuracy with far less computational complexity, while requiring fewer benign samples to establish the defense. This is achieved by designing a sample-efficient and low-complexity method for sparse recovery.}\mojan{mention that \sys{} is real-time}

% \begin{itemize}
% \item very stupid method~\cite{chen2018detecting}: \edit{from TABOR:} Chen et al. utilize contaminated training data to query the learning model. They apply clustering algorithms to the hidden layer activations to determine whether the model is infected or not. While Chen et al. ’s method demonstrates the effectiveness in de- tecting trojan backdoors, it assumes the access to the contam- inated training data as well as the internal weights. \edit{from FEBURUUS:} Nevertheless, this method requires the access to the Trojaned inputs which become unrealistic as the attackers are unlikely shipping his Trojaned examples for a user to defend.


%     \item Neural Trojans\cite{liu2017neural}. \edit{From TABOR:} utilizes anomaly detection to identify the data input that contains a trigger.
    
%     \item NIC \cite{ma2019nic}: \edit{From TABOR:} Ma et al. [35] propose to detect an input with the trigger by comparing the neurons’ activation pattern of the clean inputs and the contaminated inputs.
    
%     \item STRIP \cite{gao2019strip}: \edit{from TABOR:} Gao et al. introduce STRIP [19], a detection system that exam- ines the prediction variation and thus pinpoints the input data samples with the presence of the malicious trigger. 
    
%     \item SentiNet\cite{chou2018sentinet}: \edit{from TABOR:} Similarly, Chou et al. propose SentiNet [11], a different technical ap- proach to detect the presence of the trigger in a target input sample. Technically, SentiNet first employs an explainable AI approach [38] to highlight the features attributive to a classification result. Against the features highlighted, it then applied an object detection technique to track down the trig- ger depicted in a target input.
    
%     \item Februus~\cite{doan2019februus}: 
    
    
% \end{itemize}

% \subsection{Mitigation by training/fine-tuning}
% \edit{from TABOR:} Going beyond detecting trigger and trojan discussed above, recent research also explores techniques to disable the behavior of the backdoor in a target model. Technically speaking, the researches in this category mainly focus on three kinds of methods – (1) eliminating contaminated training data and retraining learning models (e.g. \cite{charikar2017learning, liu2017robust}); (2) trimming malicious neurons and re- calibrating the corresponding network (e.g., \cite{liu2018fine}) as well as (3) restoring a trigger from an infected model and patch the model with that trigger (i.e., \cite{wang2019neural,chen2019deepinspect}). For the first method, the state-of-the-art technique \cite{tran2018spectral} utilizes a new statistical method to examine training data and thus tracks down the training data potentially contaminated for inserting a trojan. Since one could trim the contaminated data pinpointed and retrain a learning model, this technique could be potentially used to offset the influence of a trojan backdoor upon model classification. For the second method, representative work is fine-pruning \cite{liu2018fine}. Technically speaking, it first exercises a target neural network with a large corpus of clean data sam- ples. By observing the activation of each neuron, it then cuts off the dormant neurons (i.e., those inactive in the presence of a clean input) and locally retrains the corresponding neural networks to offset the impact of the backdoor upon model classification. Different from the former two methods, the third method~\cite{wang2019neural,chen2019deepinspect} assumes that the defender cannot access the infected training data and only have clean testing data. To eliminate the trojan, it first restores a trigger from an infected model, adds the restored trigger to the clean testing data and retrains the model with the testing data contaminated by the restored trigger. In this work, we also follow this approach to patch an infected model, and as we will show later in Sec- tion §5, restoring a high-fidelity trigger will help improve the patching performance.

% \edit{from FEBURUUS}: Liu et al. \cite{liu2018fine} developed a method named Fine-Pruning
% to disable backdoors by pruning DNNs and then fine-tune the pruned network. Even though it can eliminate or weaken back- door effects, pruning the DNN will also reduce the accuracy of the system and fine-tuning will require additional re-training on the network, which make it less attractive for most DL practitioners to deploy in their systems. 

% \edit{from FEBURUUS}: Wang et al. \cite{wang2019neural} propose a novel idea of Neural Cleanse to
% detect whether the network is trojaned by reversing the Trojan triggers. Using those reversed triggers, authors use a method of unlearning to patch the performance of Trojaned DNN. However, this method exposes disadvantages to some advanced backdoor variants such as large trigger or partially poisoned network when they need to adapt their working mechanism to defend








% The research efforts in defending DNNs against Trojan attacks can be classified into three main categories: (i)~Detecting whether a model is infected with Trojans, i.e., making a binary decision about the model. (2)~Finding Trojan patterns in the input sample. (3)~Eliminating the effect of Trojan trigger, i.e., re-storing the correct classification result on the Trojaned data. Our work falls in the category of (2) and (3). 


\mojan{Though generative adversarial networks (GANs) have shown great performance in scenarios with abundant data, they are prone to failure when the number of available samples is limited~\cite{arora2017gans}.}

==> threat.tex <==
% We assume that the client buys a DNN model from the malicious party. The client therefore has access to the model weights but does not have any labeled data. The client is unaware whether the model is infected or not. The client does not have any information about possible Trojan trigger shapes. To construct the defense, we assume the client owns a small corpus of \textit{unlabeled} data\footnote{less than XXX\% of the training data size across all of our evaluations}. This is a realistic assumption as access to small amount of data is possible via the Internet. For instance, researchers have shown the possibility of data generation through generative networks for Faces~\cite{karras2017progressive}, Anime cartoon characters~\cite{jin2017towards}, image-to-image and text-to-image translation~\cite{isola2017image, zhang2017stackgan}, and online resources are publicly available\footnote{Face generation example: \url{http://www.whichfaceisreal.com/index.php}}. We consider the most generic and challenging form of Trojan attacks in which the attacker can control the trigger size, shape, and the content of the trigger. 
% \mojan{Additionally, we make no assumption about the number of attack target classes or the number of trigger patterns.}
% \sys{} mitigation is made possible in such scenarios by constructing the defense using benign unlabeled data.


% DeepInspect examines the susceptibility of the queried DNN
% against NT attacks with minimal assumptions, thus addressing
% the challenge of limited information (C2) mentioned in the
% previous section. More specifically, we assume the defender
% has the following knowledge about the inquired DNN: dimensionality of the input data, number of output classes, and the
% confidence scores of the model given an arbitrary input query.
% Furthermore, we assume the attacker has the capability of
% injecting arbitrary type and ratio poison data into the training
% set to achieve his desired attack success rate. Our strong threat
% model ensures the practical usage of DeepInspect in the realworld settings as opposed to the prior work [Wang et al., ] that
% requires a benign dataset to assist backdoor detection.

